Graphs, Ultrafilters and Colourability

Let $\beta$ be the functor from Set to CHaus which maps each discrete set X to its Stone-Cech compactification, the set $\beta$ X of ultrafilters on X. Every graph G with vertex set V naturally gives rise to a graph $\beta G$ on the set $\beta V$ of ultrafilters on V . In what follows, we interrelate the properties of G and $\beta G$. Perhaps the most striking result is that G can be finitely coloured iff $\beta G$ has no loops.

==> wrong.tex <==
\begin{proposition}
A sparse connected graph of finite girth is finite.
\end{proposition}
\begin{proof}
We can assume $|V| > 1$. By hypothesis, the adjacency relation $\rho$ is a small relation. Connectedness and finite girth imply
\[	V \times V = \bigcup_{i=1}^{n}\rho^{i}
\]
for some $n < \infty$. But each $\rho^{i}$ is a small relation, hence so is $V \times V$, forcing $|V| < \infty$.
\end{proof}
\ \\


[x] \rho_{\beta G}^{n} [y] \Rightarrow [x] \rho_{\beta (G^{n})} [y]

first consider any $x \in V$. Then $V = \cup_{n = 0}^{\gamma}x^{(n)}$, so any $\upsilon \in \beta V$ contains
one of these sets $x^{(n)}$, and so $\upsilon \in [x]^{(n)}_{\beta G}$ for some $n \leqslant \gamma$. \


Fix any $x \in V$: then by hypothesis V is a finite union of sets $x^{(n)}$: hence every $\upsilon \in \beta G$ contains one of these sets,
hence contains $y^{(1)}$ for some vertex $y$ connected to $x$.
<NOT>!!!!

